NaturalProofs: Mathematical Theorem Proving in Natural Language

Understanding and creating mathematics using natural mathematical language - the mixture of symbolic and natural language used by humans - is a challenging and important problem for driving progress in machine learning. As a step in this direction, we develop NaturalProofs, a multi-domain corpus of mathematical statements and their proofs, written in natural mathematical language. NaturalProofs unifies broad coverage, deep coverage, and low-resource mathematical sources, allowing for evaluating both in-distribution and zero-shot generalization. Using NaturalProofs, we benchmark strong neural methods on mathematical reference retrieval and generation tasks which test a system's ability to determine key results that appear in a proof. Large-scale sequence models show promise compared to classical information retrieval methods, yet their performance and out-of-domain generalization leave substantial room for improvement. NaturalProofs opens many avenues for research on challenging mathematical tasks.

==> tables/tbl_autoregressive.tex <==
\begin{table}[t]
\begin{minipage}{.33\linewidth}
\begin{center}
\begin{tabular}{ ccccc }
  \toprule
  \textbf{Init} & \textbf{Scoring} & \textbf{mAP} \\\toprule
  -- & Independent & 16.99\\
  \hline
  \xmark & Autoregressive & 17.77 \\ 
  \cmark & Autoregressive & 35.37 \\
  \xmark & Joint & 18.71 \\
  \cmark & Joint & 37.51 \\
  \bottomrule
\end{tabular}
\caption{Effects of initializing the autoregressive encoder, decoder, and reference token embeddings using the independent retrieval model, and joint vs. autoregressive in-domain retrieval performance (ProofWiki).
Initializing the joint and autoregressive models using the independent model was necessary for achieving high performance.
As a retrieval model, the autoregressive model trained for sequence generation substantially improves over the independent retrieval model, yet underperforms the joint model, which is trained specifically for retrieval.
}
\label{tbl:autoregressive-ablation}
\end{center}
\end{minipage}
\end{table}

